Double Holography of Entangled Universes

We employ double holography to examine a system of two entangled gravitating universes that live on two codimension-one branes in an asymptotically AdS$_3$ spacetime with two disjoint conformal boundaries. There are distinct brane configurations depending on the temperature of the thermofield double (TFD) state between the left and right systems. The topology transition between two branes is naturally identified with the emergence of an Einstein-Rosen bridge connecting the two entangled universes. This doubly holographic construction offers a holographic perspective on gravitational collapse and black hole formation in brane universes. Through this holographic framework, we analyze the quantum information structure of the two gravitating universes. Specifically, we calculate the mutual information between defects present in the boundary theories on the left and right sides. Furthermore, we investigate the decoupling process in the Hayden-Preskill protocol applied to the two copies of the defect field theory and discuss the interpretation of the Yoshida-Kitaev decoding protocol.

==> sections/Action.tex <==
% !TEX root = ../paper07.tex
%

%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Euclidean Action}
\begin{figure}[!]
	\centering
	\includegraphics[width=2.8in]{Integrals1.pdf}
	\quad
	\includegraphics[width=2.8in]{Integrals2.pdf}
	\caption{The contributions from the regions I, II vanish due to the cancellation between the bulk term and boundary term.}\label{fig:Integral}
\end{figure}

In this appendix, we take global AdS$_3$ as an explicit example and show that the bulk integral in Euclidean action is precisely canceled by that on the boundary. For simplicity, we will take $\ell=1$ in the following. The metric of bulk spacetime in global coordinates reads 
\begin{equation}
	 ds^2 =   (1 + R^2) d\tau^2 + \frac{dR^2 }{1+R^2} + d\phi^2 \,, 
\end{equation}
where the solution of brane profile is derived as 
\begin{equation}
	| R \cos \phi | = \frac{T_o}{\sqrt{1-T_o^2}} \equiv \alpha_o \,, \qquad \text{with} \qquad  K = 2 T_o \,. 
\end{equation}
We assume that the cut-off surface is located at 
\begin{equation}
	 R_{\rm cut} = \frac{1}{\epsilon} \,. 
\end{equation}
Furthermore, let us divide the total Euclidean action into two parts: 
\begin{equation}\label{eq:Bulk}
	I_{\rm bulk}^{\mt{E}}= - \frac{1}{16 \pi \GN} \int_{\mS} \sqrt{g}\(\mathcal{R} + \frac{2}{\ell^2} \)d^3x =  \frac{1}{4 \pi \GN} \int_{\mS} \sqrt{g} \, d^3x
\end{equation}
and 
\begin{equation}\label{eq:bdy}
	I_{\rm brane}^{\mt{E}}= - \frac{1}{8 \pi \GN} \int_{\brane } \sqrt{h}(K-T_o)d^2y =  - \frac{T_o}{8 \pi \GN} \int_{\brane } \sqrt{h} \, d^2y  = \frac{1}{2} I_{\rm GHY}\,. 
\end{equation}
Along the cut-off surface, the boundary term is given by the Gibbons–Hawking–York boundary term, namely 
\begin{equation}
	I_{\rm cut-off} =  - \frac{1}{8 \pi \GN} \int_{\rm cut-off}  K  \sqrt{h}  \, d^2y  \,. 
\end{equation}
To obtain the renormalized action, we also need to add a counterterm on the cut-off surface, \viz 
\begin{equation}
	I_{\rm ct} =  - \frac{1}{8 \pi \GN} \int_{\rm cut-off} \sqrt{h}  \, d^2y  \,. 
\end{equation}




\subsubsection{Region I} 
The intersection of the brane and cut-off surface is located at 
\begin{equation}
	R_{\rm cut} =\frac{1}{\epsilon} \,, \qquad  \phi_{\rm int} = \frac{\pi}{2} + \arcsin \(  \alpha_o \epsilon \) \,. 
\end{equation}
The bulk action  $	I_{\rm bulk}^{\mt{E}}$ reduces to 
\begin{equation}\label{eq:BulkI}
	\begin{split}
			I_{\rm bulk}^{\mt{E}} &=  \frac{1}{4 \pi \GN} \int_{\mS} \sqrt{g} \, d^3x  =   \frac{\beta}{4 \pi \GN}    \int^{\frac{\alpha_0}{\cos \phi} }_0 R \,  dR \int^{\pi}_{\phi_{\rm int} }   2 \times d \phi  \\
			&= \frac{\beta}{4 \pi \GN}    \int^{\pi}_{\phi_{\rm int} }   \(  \frac{\alpha_o}{\cos \phi} \)^2    d \phi  \\
			&= \frac{\beta}{4 \pi \GN} \cdot \alpha_o \sqrt{\frac{1}{\epsilon^2} - \alpha_o^2 } \,.
	\end{split}
\end{equation}
The volume measure on the brane is derived as 
\begin{equation}
	 \sqrt{h} =  R \sqrt{  \frac{1}{R^2   - T_o^2 (R^2+1)}  }  \,.
\end{equation}
With substituting the volume measure into the brane integral $	I_{\rm brane}^{\mt{E}}$, one can obtain the Euclidean action on the brane, \ie 
\begin{equation}
	\begin{split}
			I_{\rm brane}^{\mt{E}}  &= -    \frac{\beta \, T_o}{8 \pi \GN} \int^{\frac{1}{\epsilon}}_0  R \sqrt{  \frac{1}{R^2   - T_o^2 (R^2+1)}  } \,    dR \times 2    \\
			&= -  \frac{\beta }{4 \pi \GN} \int^{\frac{1}{\epsilon}}_0   \alpha_o R \sqrt{\frac{1}{R^2 - \alpha_o^2}}  \,    dR \,   \\
			&=-  \frac{\beta}{4 \pi \GN} \cdot \alpha_o \sqrt{\frac{1}{\epsilon^2} - \alpha_o^2 } \,.
	\end{split}
\end{equation}
As a result, we can find that the Euclidean action from region is exactly zero due to: 
\begin{equation}
	\text{Region I} : \qquad 		I_{\rm bulk}^{\mt{E}}  + I_{\rm brane}^{\mt{E}}    =0 \,. 
\end{equation}
We further note that the cancellation is precise {\bf without} taking the conformal limit $\epsilon \to 0$.

\subsubsection{Region II} 
The bulk action  $	I_{\rm bulk}^{\mt{E}}$ reads 
\begin{equation}
	\begin{split}
		I_{\rm bulk}^{\mt{E}} &=  \frac{1}{4 \pi \GN} \int_{\mS} \sqrt{g} \, d^3x  =   \frac{\beta}{4 \pi \GN}    \int^{\frac{1}{\epsilon} }_0 R \,  dR \int^{\phi_{\rm int} }_{\pi/2}   2 \times d \phi  \\
		&= \frac{\beta}{4 \pi \GN} \cdot  \frac{1}{\epsilon^2}  \arcsin (\alpha_o \epsilon)   \,.
	\end{split}
\end{equation}
The boundary term on the cut-off surface gives rise to 
\begin{equation}
	\begin{split}
			I_{\rm cut-off}  &=  - \frac{1}{8 \pi \GN} \int_{\rm cut-off}  K  \sqrt{h}  \, d^2y   \\
			 & =  - \frac{\beta }{8 \pi \GN}   \int^{\phi_{\rm int} }_{\pi/2}     2 \times (2R_{\rm cut}^2 + 1) d \phi  \\
			 &=   - \frac{\beta }{4 \pi \GN}   \( \frac{2}{\epsilon^2} +1  \)  \arcsin \(  \alpha_o \epsilon \) \,, 
	\end{split}
\end{equation}
with using 
\begin{equation}
	 \sqrt{h} =  R_{\rm cut} \sqrt{R^2_{\rm cut} +1} \,, \qquad K = \frac{2R^2_{\rm cut} +1 }{ \sqrt{h}} \,. 
 \end{equation}
The counterterm along the brane in region II is derived as 
\begin{equation}
	I_{\rm ct} =  +  \frac{1}{8 \pi \GN} \int_{\rm cut-off} \sqrt{h}  \, d^2y  =  \frac{\beta }{4 \pi \GN}    \frac{\arcsin \( \alpha_o \epsilon \) }{\epsilon}  \sqrt{\frac{1}{\epsilon^2} +1 } \,.  
\end{equation}
The total Euclidean action in region II is summarized as 
\begin{equation}
	\begin{split}
				\text{Region II } : \qquad  	I_{\rm bulk}^{\mt{E}}  + 	I_{\rm cut-off} + I_{\rm ct}  &=  \frac{\beta }{4 \pi \GN}     \cdot \arcsin \( \alpha_o \epsilon \)    \(      \frac{1}{\epsilon}\sqrt{\frac{1}{\epsilon^2} +1 } -\frac{1}{\epsilon^2} - 1    \) \\
				& \approx - \frac{\alpha_0\epsilon }{2}   \cdot  \frac{\beta }{4 \pi \GN}   \,, 
	\end{split}
 \end{equation}
which also vanishes in the limit $\epsilon \to 0$. 
\smr{I suspect that the cancellation here is not precise because we didn't count the joint term properly. The joint term between the brane surface and cut-off surface is shown as 
	\begin{equation}
		I_{\rm joint} =  -   \frac{1}{8 \pi \GN} \int  \theta  \sqrt{\gamma}  \, d\tau \times 2 \,,
	\end{equation}
with $\sqrt{\gamma}= \sqrt{1= R_{\rm cut}^2}$ and $\theta = \arccos \(  \alpha_o \sqrt{\frac{\epsilon^2+1}{\alpha_o^2 +1}} \)$. We also need to introduce a corner term in the counterterm. The simplest choice is 
\begin{equation}
I_{\rm ct}^{\rm joint} =  +  \frac{\theta_o}{8 \pi \GN} \int    \sqrt{\gamma}  \, d\tau \times 2 \,,
\end{equation}
with $\theta_o = \arccos \(   \frac{\alpha_o }{\sqrt{1+ \alpha_o^2}} \) = \arccos (T_o)$. The sum of these two joint terms produces 
\begin{equation}
	I_{\rm joint} + I_{\rm ct}^{\rm joint}  \approx + \frac{\alpha_0\epsilon }{2}   \cdot  \frac{\beta }{4 \pi \GN} + \mathcal{O}(\epsilon^3) \,. 
\end{equation}
}

\rcm{From the description above, it seems that we should include an extra counterterm at the end of the brane. However, I think the approach to joint term above is not appropriate. Rather we should consider the two portions of the cut-off surface on either side of the brane and the joint between these -- see figure \ref{fig:boundk}. The joint term then represents the contribution of a delta-function in the Gibbons-Hawking term (\ie in the extrinsic curvature of the asymptotic boundary). The question is then whether there is a divergence in the action left over after adding this joint term. If so, then we would need to add an extra counterterm at the end of the brane.}\smr{Check the additivity.}

\begin{figure}[!]
	\centering
	\includegraphics[width=3.6in]{extra.png}
	\caption{The brane will introduces a kink in the boundary.}\label{fig:boundk}
\end{figure}

\subsection{Origin of logarithmic term on the brane}
We will show that the induced action on the brane can contain the logarithmic term due to the non-vanishing of its intrinsic curvature. 



==> sections/CFTapp.tex <==
% !TEX root = ../paper07.tex
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\rcm{Equations (and in particular, signs) need to be checked throughout the following appendix.}
\smr{I corrected some signs and notations in order to match the conventions in the main text.}

To begin recall the standard treatment of evaluating the stress tensor for (holographic) CFTs. To begin, we consider a CFT coupled to a (fixed) background metric, \eg
\beq
\int D\phi\ e^{i I(\phi, g^{(0)}_{ab}) }= e^{i I_{\rm gen}(g^{(0)}_{ab})} \,.
\label{num1}
\eeq 
Above we are depicting how the path integral over the CFT degrees of freedom yields a generating function $I_{\rm gen}(g^{(0)}_{ab})$ for correlators of the CFT stress tensor, \eg
\beq
\langle T^{ab}\rangle = \frac{2}{\sqrt{-g^{(0)}}}\, \frac{\delta I_{\rm gen}}{\delta
g^{(0)}_{ab}}\,.
\label{num2}
\eeq
Of course, this generating function is a very nonlocal functional of the background metric $g^{(0)}_{ab}$. However, as presented, the problem is that the results would be UV divergent, \eg $\langle T^{ab}\rangle \sim 1/\delta^d$ where $\delta$ is a short-distance cutoff. To fix this problem, we subtract the appropriate counterterms which are local functionals of the metrc, 
\beq
\int D\phi\ e^{i \[I(\phi, g^{(0)}_{ab})- I_{\rm ct}(g^{(0)}_{ab})\]}= e^{i \[I_{\rm gen}(g^{(0)}_{ab})- I_{\rm ct}(g^{(0)}_{ab})\]} = 
e^{i I'_{\rm gen}(g^{(0)}_{ab})} \,.
\label{num3}
\eeq 
Implicitly, $\delta$ is left finite in these expressions but the counterterms ensure that the $\delta\to0$ limit yields finite results. Hence the expectation value of the stress tensor is properly given by 
\beq
\langle T^{ab}\rangle = \frac{2}{\sqrt{-g^{(0)}}}\,\lim_{\delta\to0} \frac{\delta I'_{\rm gen}}{\delta
g^{(0)}_{ab}}= \frac{2}{\sqrt{-g^{(0)}}}\,\lim_{\delta\to0} \frac{\delta \ }{\delta
g^{(0)}_{ab}}\[I_{\rm gen}- I_{\rm ct}\]\,.
\label{num4}
\eeq
Here, we have the `renormalized' stress tensor.

Of course, in the case of a holographic CFT, we can replace the path integral over the boundary CFT degrees of freedom with the path integral over the bulk degrees of freedom, in particular, the bulk metric. As indicated with the above notation, this path integral while keeping the non-normalizable mode of the metric, \ie the boundary metric $g^{(0)}_{ab}$, fixed. Further, as is standard, we assume that the latter path integral is evaluated in the usual saddle point approximation. \rcm{Could probably include some refs to this discussion.}

Now let us turn to the doubly holographic models as described in \cite{Chen:2020uac,Chen:2020hmv}. In this case, we are integrating out the bulk theory on both sides of the brane to yield two boundary CFTs, as well as a dynamical theory of gravity on the brane. In terms of the boundary theory, the corresponding path integral now takes the form
\beqa
\int D\tg\,\int D\phi_\mt{L}\,D\phi_\mt{R}&&e^{i \[ I_{\rm brane}(\tg_{ab})+\sum_i I(\phi_i, \tg_{ab}) \]}= e^{i \[ I_{\rm brane}(\tg_{ab})+\sum_i I_{{\rm{gen}},i}(\tg_{ab})\]}
\nonumber\\
&&\qquad=\int D\tg\, e^{i \[ I_{\rm brane}(\tg_{ab})+\sum_i I_{ct,i}(\tg_{ab})+\sum_i \(I_{{\rm gen},i}(\tg_{ab})-I_{{\rm{ct}},i}(\tg_{ab})\)\]}
\nn\\
&&\qquad=\int D\tg\,e^{i \[ I_{\rm grav}(\tg_{ab})+\sum_i I'_{{\rm gen},i}(\tg_{ab})\]}
\label{raz1}
\eeqa
So let's unpack the above expressions. First, we note that the expressions are written in terms of the induced metric on the brane $\tg_{ab}$, rather than the non-normalizable mode $g^{(0)}_{ab}$ which appears in the standard holographic discussion above. Further, we assume that the brane tension is tuned to be near the critical value, which yields a small UV cutoff $\delta$ and puts us in a regime where the gravitational theory on the brane is well approximated by Einstein gravity. Of course, in contrast to the above discussion, the cutoff $\delta$ remains finite throughout.

Now, the brane has an intrinsic action which typically takes the form of the tension or worldvolume term
\begin{equation}\label{bran1}
	I_{\mB}=- \frac{T_o}{4 \pi \GN }\,\int d^dx\,\sqrt{-\tg}\,,
\end{equation}
however, we may also add various DGP terms, as described in \cite{Chen:2020uac,Chen:2020hmv}. Now as noted in the preceding references, the `divergences' generated by the integrating out the boundary CFTs or the bulk metrics on either side of the brane are what induces the gravitational action on the brane. That is, the gravitational brane action is given by
\begin{equation}\label{grav1}
	I_{\rm grav}=I_{\mB} + \sum_i I_{{\rm{ct}},i}\,,
\end{equation}
where we are distinguishing the contributions coming from the two CFTs. However, these UV divergences are all local functionals of the brane metric $\tg_{ab}$ and so they will be identical for the two theories.\footnote{Implicitly, this conclusion arises because the bulk theory (in particular, the cosmological constant) is identical on either side of the brane. However, if we generalized the discussion so that the bulk theories on either side of the brane were different (\eg $\ell_1\ne\ell_2$), this would change the nature of the two boundary CFTs. In this case, as a functional of the brane metric, the form of the divergences would be the same, however, the precise coefficients of the individual terms need not be the same.}

Lastly, in eq.~\reef{raz1}, we add and subtract the counterterm action and so the argument in the exponential is identical in all three lines. We have introduced the counterterm action as an accounting device to rearrange the contributions in an interpretable way. In particular, apart from the gravitational action \reef{grav1}, we have identified the generating functions
\beq
I'_{{\rm{gen}},i}=I_{{\rm{gen}},i}-I_{{\rm{ct}},i}\,.
\label{CFT1}
\eeq
These are identical to the expressions derived in the standard holographic approach and would yield, for instance, the expectation value of the CFT stress tensor in the limit $\delta\to0$. Here we interpret the result
\beq
\langle T_i^{ab}\rangle = \frac{2}{\sqrt{-\tg}}\, \frac{\delta I'_{{\rm{gen}},i}}{\delta
\tg_{ab}}
\label{CFT2}
\eeq
as the expectation value in the CFT with a finite cutoff. That is, if yields the expected result for the CFT plus small corrections which vanish in the limit $\delta\to0$. Of course, these expectation values act as a source in the gravitational equations of motion on the brane. 

\rcm{With this construction, we seem to identify an independent $I'_{\rm gen}$ for each of the two CFTs. Hence we would find the two stress tensors are uncoupled/uncorrelated, \eg
\beq
\langle T_\mt{L}^{ab}\, T_\mt{R}^{ab}\rangle=\langle T_\mt{L}^{ab}\rangle\,\langle T_\mt{R}^{ab}\rangle\,.
\label{curious}
\eeq 
This seems curious and possibly incorrect???}\smr{I guess the reason is that we generally cannot uniquely decompose the counterterm $\sum_{i} I_{ct,i}$ of eq.~\eqref{grav1} into two independent parts.}

Let us turn to the situation discussed in the main text, namely, with $d=2$. In this case, the counterterm action contains a single term
\begin{equation}\label{count1}
	I_{{\rm{ct}},i}=\frac{1}{8\pi\GN\,\ell}\int d^2x \,\sqrt{-\tg} =
	\frac{1}{16\pi G_\mt{eff}}\int d^2x\,\sqrt{-\tg} \,\frac2{\ell^2}  \,,
\end{equation}
where $\GN$ and $G_\mt{eff}=\GN /\ell$ are the Newton's constants for the bulk and brane theories \cite{Chen:2020uac,Chen:2020hmv,Grimaldi:2022suv}.\footnote{The Einstein term on the brane is topological and so the definition of $G_\mt{eff}$ is a convention, \eg \cite{Grimaldi:2022suv}.} This term combines with the tension term to yield the effective cosmological constant term
\begin{equation}\label{const2}
	\frac{1}{16\pi G_\mt{eff}}\int d^2x\,\sqrt{-\tg}\,\frac{2}{\ell_\mt{eff}^2}=\frac{1}{4\pi\GN}\int d^2x\,\sqrt{-\tg} \(\frac{1}{\ell}-T_o\)\,.
\end{equation}
In fact, the gravitational action really only has a cosmological constant term and so the gravitational equation of motion becomes
\begin{equation}\label{eom1}
	\begin{split}
		0&=\frac1{8\pi G_\mt{eff}}\,\frac{1}{\ell_\mt{eff}^2} \,\tg_{ab}+\langle T_{ab}^{(1)}   \rangle+
		\langle T_{ab}^{(2)}\rangle  \\
		&=\frac{1}{4\pi \GN}\(\frac{1}{\ell}-T_o\)\tg_{ab}+ \langle T_{ab}^{(1)}   \rangle+
		\langle T_{ab}^{(2)}\rangle\,.
	\end{split}
\end{equation}
To connect to the discussion in \cite{Chen:2020uac,Chen:2020hmv,Grimaldi:2022suv}, the contribution of the stress tensors here corresponds to the contribution coming from finite terms in the gravitational action presented there, \ie the $R\log R$ term and higher powers of the curvature.


Now let us compare to the discussion in \cite{Kawamoto:2023wzj}. There the total action on the brane takes the simple form
\begin{equation}\label{simp2}
	I_{\rm brane}=\frac{1}{8\pi\GN} \int d^2x\,\sqrt{-\tg}\(K^{(1)}+K^{(2)}-2T_o\)\,,
\end{equation}
and the corresponding boundary equation of motion corresponds to the Israel junction condition
\beq
0=\frac{1}{8\pi\GN} \(K_{ab}^{(1)} + K_{ab}^{(2)} -  \( K^{(1)}+ K^{(2)}- 2 T_o \) \tg_{ab} \) \,.
\label{eom2}
\eeq
Hence if we compare eqs.~\reef{eom1} and \reef{eom2}, it would seem that we can identify
\begin{equation}\label{stress9}
	\langle T_{ab}^{(i)}  \rangle=-\frac{1}{8\pi\GN}\(K^{(i)}_{ab}- K^{(i)}\tg_{ab}+\frac{1}{\ell}\tg_{ab}\)\,.
\end{equation}
\smr{Have corrected some signs in the above equations.}
This corresponds to the quasilocal stress tensor appearing in the standard holographic setup, as defined by \cite{Balasubramanian:1999re} -- except that we do not take the $\delta\to0$ limit.  \rcm{Except I seem to have mess up some signs somewhere?? Perhaps I may have defined my extrinsic curvature with the opposite sign, \ie $K_{ab}=-\Theta_{ab}$??} In general, the latter is given by
\begin{equation}\label{stress8}
	\langle T^{ab}\rangle=+ \frac{2}{\sqrt{-\tg}}\frac{\delta I_{\rm tot}}{\delta \tg_{ab}} =-\frac{1}{8\pi\GN}\(K^{ab}-K\,\tg^{ab}\) + \frac{2}{\sqrt{-\tg}}\frac{\delta I_{\rm ct}}{\delta \tg_{ab}} \,.
\end{equation}
\rcm{Note that I also seem to have flipped the sign of the counterterm action.}\smr{I think I have corrected the sign problems in this appendix.}

==> sections/notations.tex <==
% !TEX root = ../paper07.tex
%

%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%

Let us fix the conventions here. Table of notation and conventions (I am using): 

\smr{I change the notation of tension to $T_o$ as previous papers. It is also useful to use the dimensionless tension $\mathcal{T}_o = T_o \ell$.} \rcm{We are really not using the same conventions for $T_o$ as in the `made easy' papers. May be it doesn't matter.}

%\newpage
	\begin{center}
		\renewcommand*{\arraystretch}{1.25}
		\begin{longtable}{|l|l|l|}
			\hline
			\textbf{Symbol} & \textbf{Meaning} \\
			\hline
			$c=c_1=c_2$ & Central charge of the boundary CFTs (between the defects) \\
			$L_1, L_2$ & Length of the corresponding boundary regions\\
			$S_{\rm bdy} =\log g $ &   Boundary entropy \\
			$ \epsilon=L \, \delta $ &  UV cut-off in DCFT \\
			$L_{\rm bdy}= L_1+ L_2$ & Total length of the left/right boundary circle\\
			$T_{\mt{DFCT}}$ & Temperature of the boundary defect field theory\\
			\hline
			\hline
			$\tau \equiv T_{\mt{DCFT}} \(   L_1 +   L_2 \)$ &  Dimensionless total size\\ 
			$\gamma \equiv  \frac{L_1}{L_2}$  &  Dimensionless ratio of the sizes of two boundary regions\\
			\hline
			\hline
			$\ell=\ell_1= \ell_2$ & AdS radius of the two bulk AdS$_3$ spacetimes\\
			$\mathcal{R}$ &   Ricci scalar of bulk AdS spacetime \\
			$T_o$ &   Tension of the brane (for one side), $[T_o]=[\frac{1}{\ell}]$\\
			$K_{ij}, K = K_i^i$ &   Extrinsic curvature of the brane  (for one side), $[K]=[\frac{1}{\ell}]$\\
			$\log g =  \frac{c }{6}  \log \(   \sqrt{   \frac{ 1+T_o\ell}{1-T_o\ell}  }\)   $ &   Boundary entropy in terms of the tension of the brane in one side\\
			$(t, r , \phi),(t_i, r_i, \phi_i)$ &   bulk coordinates in $\mS_1, \mS_2$ \\
			$(\tp, \zp , \xp)$ &   Poincar\'e coordinates \\
			$S_{\mt{EE}}$ &   (Holographic) entanglement entropy\\
			\hline
			\hline
				$\ellB$ & AdS radius of the brane geometry\\
			$h_{ij}$ &  Induced metric on the two-dimensional brane(s)\\
			$R[h]$ &   Ricci scalar of the brane geometry with induced metric $h_{ij}$ \\
			\hline
		\end{longtable}
	\end{center}





%%%%%%%%%%%%%%%%%%%%%%%
